Learning-based Models for Vulnerability Detection: An Extensive Study

Though many deep learning-based models have made great progress in vulnerability detection, we have no good understanding of these models, which limits the further advancement of model capability, understanding of the mechanism of model detection, and efficiency and safety of practical application of models. In this paper, we extensively and comprehensively investigate two types of state-of-the-art learning-based approaches (sequence-based and graph-based) by conducting experiments on a recently built large-scale dataset. We investigate seven research questions from five dimensions, namely model capabilities, model interpretation, model stability, ease of use of model, and model economy. We experimentally demonstrate the priority of sequence-based models and the limited abilities of both LLM (ChatGPT) and graph-based models. We explore the types of vulnerability that learning-based models skilled in and reveal the instability of the models though the input is subtlely semantical-equivalently changed. We empirically explain what the models have learned. We summarize the pre-processing as well as requirements for easily using the models. Finally, we initially induce the vital information for economically and safely practical usage of these models.

==> sections/dataset-backup.tex <==
\subsection{Dataset Construction}

% \chao{introduction to our extended dataset, which should include what are the new contributions of our dataset and how we build such a dataset }


    
\sly{In order to fully evaluate the performance of LLM and graph models for real-world vulnerability detection, we constructed a new high-quality, data-rich, multi-dimensional C/C++ dataset named \textbf{Vul4C}.
Although there are some existing datasets for vulnerability detection that have been used in recent research, those have various shortcomings. 
For instance, SARD\cite{sard} used by SeSyVR\cite{li2021sysevr} and VulDeeLocator\cite{li2021vuldeelocator} artificially synthesize vulnerable code using known vulnerable patterns, which are too simple to reflect complex and implicit vulnerability patterns in the real world. 
Zhou et al. curated Devign\cite{zhou2019devign} dataset from 4 popular open-source projects, they extract the vulnerable function and clean function from the previous and current version of the vulnerable-fix commits. As a result, the ratio of vulnerable and non-vulnerable examples is approximately 1:1, which does not reflect the true distribution of vulnerable code.
Chakraborty et al.\cite{chakraborty2021deep} curate a more robust and comprehensive real world dataset ReVeal from two open-source repository (i.e. Linux Kernel and Chromium). Despite the abundance of reported vulnerabilities in both projects, it is worth noting that these vulnerabilities do not encompass the entirety of the diverse and widespread range of vulnerability types in the realistic scenarios. 
Recently Fan et al.\cite{fan2020ac} curated BigVul dataset, which scraped the CVE Details database and collected CVE entries covering the period from 2003 to 2019, resulting 3,754 code vulnerabilities spanning 91 different vulnerability types. 
However their dataset lacks regular updates, with an additional 70,610 CVE records added so far in 2020 as of the first quarter of 2023. 
Upon a thorough manual analysis of BigVul, we have discovered several shortcomings in its quality. Specifically, we have found that the extracted functions are incomplete, multiple functions are erroneously merged into one, and some information is missing (e.g. CWE ID, commit message).
}

\sly{
In this paper, to address the aforementioned problems. We crawl data from more open-source repositories, using sophisticated filtering methods to improve the quality of the collected data. Furthermore, we employing advanced techniques to extract functions. Besides the raw functions collection, we also provide additional dimensions of function information, including the abstracted functions and Joern graphs, from which the AST and CFG of the function can be obtained. These supplementary information aim to avoid the need for people to implement another set of logic to extract these information, and facilitate further research in this field. Table \ref{tab:vul4c} presents the comparative statistical information between Vul4C and BigVul, and we describe the detailed procedures below.
}

\sly{
\textbf{Data Source} The National Vulnerability Database(NVD)\cite{nvd} is a public resource maintained by NIST to collect, organize and distribute information on security vulnerabilities in software products, which is a good starting-point for collecting a high-quality, comprehensive dataset for vulnerability detection. We scraped the all available Common Vulnerabilities and Exposures(CVE)\cite{cve} entries from the dataset in JSON format provided by the NVD.
By collecting these CVE entries, we can extract valuable descriptive information such as the CVE IDs, CVE summary, CVSS severity scores, and reference links to relevant products or patches for fixing the vulnerabilities.
Then we dug into the vulnerability fix commits for each CVE.
For each vulnerability fix commit, we follow Chakraborty et al.'s\cite{chakraborty2021deep} approach of annotating previous version of modified functions in the commit (i.e. the parent commit) as vulnerable, while considering the current version of the modified function as non-vulnerable. 
Moreover, those functions that remain unchanged are annotated as non-vulnerable.
In summary we need to download metadata and modified files for the vulnerability fix commit, and the corresponding parent commit.
Through manual analysis of the referenced commit links in CVE entries, we identified 17 Git code hosting platform from 349 websites that had referenced the CVE entries more than 100 times. 
The web-based code hosting platforms can be categorized into five main categories: Github, GitLab, GitWeb, CGit, and Gitiles.
We implement logic to download commits for each platform individually, while also ensuring the integrity of the downloaded commit. For example, we utilize the official GitHub API to handle downloads from GitHub, and employ crawler for GitWeb to traverse the commit's metadata and extract the download path of the files.
Ultimately, we successfully obtained 8,334 commits from 198994 CVE entries through the download process.
}

\sly{
\textbf{Function Extract}
Our dataset aims to collect function-level vulnerabilities in C/C++ code, which constitute the vast majority of vulnerabilities recorded in the NVD database.
For files included in the commit, we gather C/C++ related source code and headers based on their file extensions, while filtering out any other files.
In the next step, we need to separate the functions in the file. 
Existing datasets are implemented through predefined rules or by using regular expression tools like lizard. However, these methods have limitations due to their simplicity. 
For example, regular expressions cannot fully represent the complex syntax rules of the C-like language. 
As a result, these methods may result in the extraction of incomplete functions or the incorrect separation of multiple functions into a single function.
We used the syntax rule-based parser tree-sitter to separate functions, and on top of that extended the syntax rules to identify more macro modifiers frequently used by popular open source projects, such as the macro modifier \textit{\_\_init} defined in Linux.
Furthermore, we temporarily remove the macros from the code before parsing, which allows the parser to effectively and accurately separate the functions without the interference of macros.
% We ended up with \textcolor{red}{xxx} previous and current version of the function from \textcolor{red}{xxx} commits with code changes. 
% Furthermore, we additionally extract \textcolor{red}{xxx} functions that remained unchanged between the previous and current version of the commits.
}

\sly{
\textbf{Post-processing}
At this stage, we perform filtering on the dataset and enrich the information within it. 
Specifically, we employ three filtering strategies to further enhance the quality of the data:
1) Filtering functions with more than 5,000 lines of code. Most of these functions are automatically generated by lexer parsers such as Antlr and Yacc.
2) Removing newly added functions in commits. This is because we cannot determine whether they contain vulnerabilities.
3) Filtering functions with more than 1,000 lines of code changes. These functions may involve code refactoring. To avoid excessive complexity and maintain the significance of subsequent analysis, we have filtered out large-scale code changes.
Existing datasets solely provide the string representation of functions, disregarding other dimensional information of functions that numerous deep learning-based vulnerability detection models rely on. For example, 
Graph-based\cite{chakraborty2021deep,zhou2019devign,li2021vulnerability} models leverage function's AST, CPG\cite{cpg-yamaguchi2014modeling}, and other graph structures to effectively capture the syntactic and semantic characteristics of code. Token-based sequence models address the problem of vocabulary explosion by abstracting specific elements, such as substituting variable names with symbolic names like "VAR" \cite{li2021sysevr}. Vul4C, in contrast, addresses these limitations by offering more comprehensive dimensional information. 
Not only does this approach liberate researchers from the repetitive task of implementing the necessary logic, but by incorporating a fixed version of the data, it facilitates a fair comparison and evaluation of various vulnerability detection models.
Consequently, Vul4C provides information on the four dimensions of the function, which include: 
1) Function signature: This includes the function name, a comprehensive list of arguments with their respective names and types, and the return type of the function.
2) Abstracted function: Nine levels of granularity abstraction (e.g. FUNC, VAR, STRING) and corresponding mappings.
3) Parsed Function by Joern: The \textit{Joern}\cite{joern} tool statically parses functions, generating graph representations that offer insights into their structure and dependencies. These representations include Abstract Syntax Trees (AST), Program Dependence Graphs (PDG)\cite{cpg-ferrante1987program}, and more.
4) Code changes: Details of function changes are generated using the \textit{diff}\cite{git} tool, including line level modifications, additions and deletions.}

\sly{
The Vul4C dataset initially collected 8,234 raw commits based on the CVE entries recorded in the NVD dataset. After the Function Extract and Post-processing phases, we ended up with 6,437 commits covering 736 different projects. In total, from the 8,795 modified files, we extracted approximately 14,000 vulnerable functions across 159 CWE types, as well as 377,000 functions without vulnerabilities.
We distribute Vul4C and its build scripts for future research.
}

\begin{table}[htbp]
  \centering
  \caption{Descriptive statistics for \datasetname and BigVul}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|r|r}
    \toprule
 & Vul4C & BigVul\\
\midrule

Number of Projects & 736 & 310\\
Number of CVE IDs & 5714 & 3539\\
Date range of crawled CVEs & 2013/01-2023/04 & 2013/01-2019/03 \\
Number of CWE IDs & 159 & 92\\
Number of Commits & 6437 & 4058\\
\makecell{Number of \\ Crawled Code Hosting Platform }  &  17 & 2 \\
Number of Vul/Non-Vul Function & 14216/377185 & 10900/177736  \\ 
Function Extract Strategy/(Quality)  & Tree-sitter(High) &  Lizard(Low) \\ 
Dimensions of Information & 
% \makecell{CVSS,Diff info, Commit structure \\ \textit{Nine-granularity} abstraction \\ \textit{Joern} graph,function signature}
% & CVSS,Diff info \\
6 & 2 \\
Code Availability & Full & Partial \\
\bottomrule
\end{tabular}}
\label{tab:vul4c}
\end{table}



==> sections/dataset-old.tex <==
\subsection{Dataset Construction}

% \chao{introduction to our extended dataset, which should include what are the new contributions of our dataset and how we build such a dataset }


Though many vulnerability-related datasets have been proposed, there are still some limitations that impact the verification of proposed models, including (1) \textit{unreal vulnerability} (i.e., SARD~\cite{sard} is artificially synthesized), (2) \textit{unreal data distribution} (i.e., balanced distribution in Devign~\cite{zhou2019devign}), (3) \textit{limited diversity} (i.e., limited projects and vulnerability types in ReVeal~\cite{chakraborty2021deep}), (4) \textit{limited newly disclosed vulnerabilities} (i.e., no updated to Big-Vul~\cite{fan2020ac} covering the period only from 2003 to 2019), and (5) \textit{low-quality of dataset} (i.e., incomplete function, erroneously merged functions, missed commit message in Big-Vul~\cite{fan2020ac}).


    
% \sly{In order to fully evaluate the performance of LLM and graph models for real-world vulnerability detection, we constructed a new high-quality, data-rich, multi-dimensional C/C++ dataset named \textbf{Vul4C}.
% Although there are some existing datasets for vulnerability detection that have been used in recent research, those have various shortcomings. 
% For instance, SARD\cite{sard} used by SeSyVR\cite{li2021sysevr} and VulDeeLocator\cite{li2021vuldeelocator} artificially synthesize vulnerable code using known vulnerable patterns, which are too simple to reflect complex and implicit vulnerability patterns in the real world. 
% % Zhou et al. curated Devign\cite{zhou2019devign} dataset from 4 popular open-source projects, they extract the vulnerable function and clean function from the previous and current version of the vulnerable-fix commits. As a result, the ratio of vulnerable and non-vulnerable examples is approximately 1:1, which does not reflect the true distribution of vulnerable code.
% Zhou et al. curated Devign\cite{zhou2019devign} dataset from 4 popular open-source projects, the ratio of vulnerable and non-vulnerable examples is approximately 1:1, which does not reflect the true distribution of vulnerable code.
% % Chakraborty et al.\cite{chakraborty2021deep} curate a more robust and comprehensive real world dataset ReVeal from two open-source repository (i.e. Linux Kernel and Chromium). Despite the abundance of reported vulnerabilities in both projects, it is worth noting that these vulnerabilities do not encompass the entirety of the diverse and widespread range of vulnerability types in the realistic scenarios. 
% Chakraborty et al.\cite{chakraborty2021deep} curate a more robust real world dataset ReVeal from two open-source repository (i.e. Linux Kernel and Chromium). 
% Despite the abundance of reported vulnerabilities in both projects, it is worth noting that these vulnerabilities do not encompass the entirety of the diverse and widespread range of vulnerability types in the realistic scenarios. 
% % Recently Fan et al.\cite{fan2020ac} curated BigVul dataset, which scraped the CVE Details database and collected CVEs  covering the period from 2003 to 2019, resulting 3,754 code vulnerabilities spanning 91 different vulnerability types. 
% Recently Fan et al.\cite{fan2020ac} curated BigVul dataset, which scraped the CVE Details database and collected CVEs covering the period from 2003 to 2019.
% However their dataset lacks regular updates, with an additional 70,610 CVEs added so far in 2020 as of the first quarter of 2023. 
% % Upon a thorough manual analysis of BigVul, we have discovered several shortcomings in its quality. Specifically, we have found that the extracted functions are incomplete, multiple functions are erroneously merged into one, and some information is missing (e.g. CWE ID, commit message).
% Upon a thorough manual analysis of BigVul, we have discovered several shortcomings in its quality. Specifically, we have found that the extracted functions are incomplete, multiple functions are erroneously merged into one, and some information is missing (e.g. commit message).
% }


% \sly{In order to fully evaluate the performance of LLM and graph models for real-world vulnerability detection, 


To address the aforementioned issues, we constructed a new high-quality, data-rich, multi-dimensional C/C++ dataset named \datasetname by crawling data from more open-source repositories, adopting sophisticated filtering strategies  to improve the quality, and employing advanced techniques to extract complete functions.
Besides collecting the raw functions, we additionally provide more dimension information of function, including the abstracted function and kinds of graphs, from which the AST and CFG of the function can be obtained. 
This supplementary information facilitates further research in this field. 
Table \ref{tab:vul4c} presents the comparative statistical information between \datasetname and Big-Vul, and the collection procedures are briefly described as follows.

\begin{table}[htbp]
\vspace{-0.3cm}
  \centering
  \caption{Descriptive statistics for \datasetname and Big-Vul}
    \resizebox{\linewidth}{!}
    {
    \begin{tabular}{l|r|r}
    \toprule
 & \textbf{\datasetname} & \textbf{Big-Vul}\\
\midrule

Number of Projects & 736 & 310\\
Number of CVE IDs & 5,714 & 3,539\\
Date range of crawled CVEs & 2013/01$\sim$2023/04 & 2013/01$\sim$2019/03 \\
Number of CWE IDs & 159 & 92\\
Number of Commits & 6,437 & 4,058\\
Number of Crawled Code Hosting Platform   &  17 & 2 \\
Number of Vul/Non-Vul Function & 14,216/377,185 & 10,900/177,736  \\ 
Function Extract Strategy/(Quality)  & Tree-sitter/(High) &  Lizard/(Low) \\ 
Dimensions of Information & 
% \makecell{CVSS,Diff info, Commit structure \\ \textit{Nine-granularity} abstraction \\ \textit{Joern} graph,function signature}
% & CVSS,Diff info \\
6 & 2 \\
Code Availability & Full & Partial \\
\bottomrule
\end{tabular}}
\vspace{-0.3cm}
\label{tab:vul4c}
\end{table}





% \sly{
% In this paper, to address the aforementioned problems. We crawl data from more open-source repositories, using sophisticated filtering methods to improve the quality of the collected data. Furthermore, we employing advanced techniques to extract functions. Besides the raw functions collection, we also provide additional dimensions of function information, including the abstracted functions and Joern graphs, from which the AST and CFG of the function can be obtained. These supplementary information 
% % aim to avoid the need for people to implement another set of logic to extract these information, and 
% facilitate further research in this field. Table \ref{tab:vul4c} presents the comparative statistical information between Vul4C and BigVul, and we describe the detailed procedures below.
% }


\textbf{Data Source}. 
The National Vulnerability Database (NVD)~\cite{nvd} is a public resource maintained by NIST to collect, organize, and distribute information on security vulnerabilities in software products, which is a good starting point for collecting a high-quality, comprehensive dataset for vulnerability detection. 
We crawl all available Common Vulnerabilities and Exposures(CVE)~\cite{cve} provided by the NVD, which contains valuable descriptive information, including CVSS scores, and reference links to relevant products or patches for fixing the vulnerabilities.
Then we dig into the vulnerability fix commits for each CVE.
For each commit, following previous work~\cite{chakraborty2021deep}, we  annotate the previous version of modified functions in the commit (i.e. the parent commit) as vulnerable, and treat the current version of the modified function as non-vulnerable. 
Moreover, those functions that remain unchanged are also annotated as non-vulnerable.
In summary, we collect 17 Git-based code hosting platforms from 349 websites that had referenced the CVEs more than 100 times. 
The web-based code hosting platforms can be categorized into five main categories: GitHub, GitLab, GitWeb, CGit, and Gitiles.
Ultimately, we successfully obtain 8,334 commits from 198,994 CVEs.




% \sly{
% \textbf{Data Source} The National Vulnerability Database(NVD)\cite{nvd} is a public resource maintained by NIST to collect, organize and distribute information on security vulnerabilities in software products, which is a good starting-point for collecting a high-quality, comprehensive dataset for vulnerability detection. We scraped the all available Common Vulnerabilities and Exposures(CVE)\cite{cve} 
% % from the dataset in JSON format 
% provided by the NVD.
% % By collecting these CVEs ,
% % we can extract valuable descriptive information such as the CVE IDs, CVE summary, CVSS severity scores, and reference links to relevant products or patches for fixing the vulnerabilities.
% % These CVEs provide valuable descriptive information, including CVE IDs, CVE summaries, CVSS scores, and reference links to relevant products or patches for fixing the vulnerabilities.
% These CVEs provide valuable descriptive information, including CVSS scores, and reference links to relevant products or patches for fixing the vulnerabilities.
% Then we dug into the vulnerability fix commits for each CVE.
% % For each vulnerability fix commit, we follow Chakraborty et al.'s\cite{chakraborty2021deep} approach of annotating previous version of modified functions in the commit (i.e. the parent commit) as vulnerable, while considering the current version of the modified function as non-vulnerable. 
% For each commit, we follow Chakraborty et al.'s\cite{chakraborty2021deep} approach of annotating previous version of modified functions in the commit (i.e. the parent commit) as vulnerable, while considering the current version of the modified function as non-vulnerable. 
% Moreover, those functions that remain unchanged are annotated as non-vulnerable.
% In summary we need to download metadata and modified files for the vulnerability fix commit, and the corresponding parent commit.
% Through manual analysis of the referenced commit links in CVEs , we identified 17 Git code hosting platform from 349 websites that had referenced the CVEs  more than 100 times. 
% The web-based code hosting platforms can be categorized into five main categories: Github, GitLab, GitWeb, CGit, and Gitiles.
% We implement logic to download commits for each platform individually
% % , while also ensuring the integrity of the downloaded commit. For example, we utilize the official GitHub API to handle downloads from GitHub, and employ crawler for GitWeb to traverse the commit's metadata and extract the download path of the files.
% Ultimately, we successfully obtained 8,334 commits from 198994 CVEs  through the download process.
% }



\textbf{Function Extraction}.
Our dataset aims to collect function-level vulnerabilities in C/C++ language, which constitute the vast majority of vulnerabilities recorded in the NVD database.
Firstly, for files included in the commit, we only gather C/C++ related source codes and headers based on their file extensions.
Then, we separate the functions inside each file, which is the key component to ensure the quality and completeness of extracted functions.
Previous simply extract functions by using regular expression-based tools (e.g., lizard) or predefined rules, which  cannot fully represent the complex syntax rules of the C-like language and consequently lead to incomplete or incorrect functions.
Accordingly, we adopt the syntax rule-based parser Tree-sitter~\cite{tree-sitter} to separate functions and extend the syntax rules to identify more macros used by popular open source projects, such as the macro  ``\textit{\_\_init}'' defined in Linux.












% \sly{
% \textbf{Function Extract}
% Our dataset aims to collect function-level vulnerabilities in C/C++ language, which constitute the vast majority of vulnerabilities recorded in the NVD database.
% For files included in the commit, we gather C/C++ related source code and headers based on their file extensions, while filtering out  other files.
% In the next step, we need to separate the functions in the file. 
% Existing datasets are implemented through predefined rules or by using regular expression tools like lizard. However, these methods have limitations due to their simplicity, which cannot fully represent the complex syntax rules of the C-like language.
% % For example, regular expressions cannot fully represent the complex syntax rules of the C-like language. 
% As a result, these methods may result in the extraction of incomplete functions or the incorrect separation of multiple functions into a single function.
% % We used the syntax rule-based parser Tree-sitter\cite{tree-sitter} to separate functions, and on top of that extended the syntax rules to identify more macro modifiers frequently used by popular open source projects, such as the macro modifier \textit{\_\_init} defined in Linux.
% We used the syntax rule-based parser Tree-sitter\cite{tree-sitter} to separate functions, and extend the syntax rules to identify more macros used by popular open source projects, such as the macro  \textit{\_\_init} defined in Linux.
% % Furthermore, we temporarily remove the macros from the code before parsing, which allows the parser to effectively and accurately separate the functions without the interference of macros.
% % We ended up with \textcolor{red}{xxx} previous and current version of the function from \textcolor{red}{xxx} commits with code changes. 
% % Furthermore, we additionally extract \textcolor{red}{xxx} functions that remained unchanged between the previous and current version of the commits.
% }



\textbf{Data Enriching}.
We aim to enrich the data information by providing more types of representation.
For example, graph representation is tedious work but extremely required by graph-based models~\cite{chakraborty2021deep,zhou2019devign,li2021vulnerability}.
``Abstraction'' (e.g., substituting variable names with symbolic names like ``VAR''~\cite{li2021sysevr}) is also needed by token-based sequence models to address the problem of vocabulary explosion.
To avoid the bias in our enriched dataset, we set up three filtering criteria for further improving the dataset quality:
(1) filtering functions with more than 5,000 lines of code since  most of these functions are automatically generated by lexer parsers (e.g., Antlr and Yacc);
(2) removing newly added functions in commits since we cannot determine whether they contain vulnerabilities; 
(3) filtering functions with more than 1,000 lines of code changes since they may involve code refactoring.
Eventually, \datasetname provides information on the four dimensions of the function: 
(1) \textit{Function Signature}: includes the function name and its corresponding parameters list.
(2) \textit{Abstracted Function}: provides nine types of granularity abstraction (e.g., FUNC, VAR, STRING, etc.) and corresponding mappings.
(3) \textit{Parsed Function}: means the functions with graph representations statically parsed by \textit{Joern}~\cite{joern}.
(4) \textit{Code Changes}: include the details of function changes generated by \textit{diff} tool~\cite{git}.



% \sly{
% \textbf{Post-processing}
% At this stage, we perform filtering on the dataset and enrich the information within it. 
% Specifically, we employ three filtering strategies to further enhance the quality of the data:
% 1) Filtering functions with more than 5,000 lines of code. Most of these functions are automatically generated by lexer parsers such as Antlr and Yacc.
% 2) Removing newly added functions in commits. This is because we cannot determine whether they contain vulnerabilities.
% 3) Filtering functions with more than 1,000 lines of code changes. These functions may involve code refactoring.
% % To avoid excessive complexity and maintain the significance of subsequent analysis, we have filtered out large-scale code changes.
% Existing datasets solely provide the string representation of functions, disregarding other dimensional information of functions that numerous deep learning-based vulnerability detection models rely on. For example, 
% % Graph-based\cite{chakraborty2021deep,zhou2019devign,li2021vulnerability} models leverage function's AST, CPG\cite{cpg-yamaguchi2014modeling}, and other graph structures to effectively capture the syntactic and semantic characteristics of code. Token-based sequence models address the problem of vocabulary explosion by abstracting specific elements, such as substituting variable names with symbolic names like "VAR" \cite{li2021sysevr}. Vul4C, in contrast, addresses these limitations by offering more comprehensive dimensional information. 
% Graph-based\cite{chakraborty2021deep,zhou2019devign,li2021vulnerability} models leverage function's AST, CPG\cite{cpg-yamaguchi2014modeling}, to effectively capture the syntactic and semantic of code. Token-based sequence models address the problem of vocabulary explosion by abstracting specific elements, such as substituting variable names with symbolic names like "VAR" \cite{li2021sysevr}. Vul4C, in contrast, addresses these limitations by offering more comprehensive dimensional information. 
% Not only does this approach liberate researchers from the repetitive task of implementing the necessary logic, but by incorporating a fixed version of the data, it facilitates a fair comparison and evaluation of various vulnerability detection models.
% Consequently, Vul4C provides information on the four dimensions of the function, which include: 
% % 1) Function signature: This includes the function name, a comprehensive list of arguments with their respective names and types, and the return type of the function.
% 1) Function signature: This includes the function name and parameter list.
% 2) Abstracted function: Nine levels of granularity abstraction (e.g. FUNC, VAR, STRING) and corresponding mappings.
% % 3) Parsed Function by Joern: The \textit{Joern}\cite{joern} tool statically parses functions, generating graph representations that offer insights into their structure and dependencies. These representations include Abstract Syntax Trees (AST), Program Dependence Graphs (PDG)\cite{cpg-ferrante1987program}, and more.
% 3) Parsed Function by Joern: The \textit{Joern}\cite{joern} tool statically parses functions, generating graph representations.
% % 4) Code changes: Details of function changes are generated using the \textit{diff}\cite{git} tool, including line level modifications, additions and deletions.
% 4) Code changes: Details of function changes are generated using the \textit{diff}\cite{git} tool.
% }

% \sly{
% The Vul4C dataset initially collected 8,234 raw commits based on the CVEs  recorded in the NVD dataset. After the Function Extract and Post-processing phases, we ended up with 6,437 commits covering 736 different projects. In total, from the 8,795 modified files, we extracted approximately 14,000 vulnerable functions across 159 CWE types, as well as 377,000 functions without vulnerabilities.
% We distribute Vul4C and its build scripts for future research.
% }




